Understanding Fault Scenarios and Impacts through Fault Injection Experiments in Cielo

We present a set of fault injection experiments performed on the ACES (LANL/SNL) Cray XE supercomputer Cielo. We use this experimental campaign to improve the understanding of failure causes and propagation that we observed in the field failure data analysis of NCSA's Blue Waters. We use the data collected from the logs and from network performance counter data 1) to characterize the fault-error-failure sequence and recovery mechanisms in the Gemini network and in the Cray compute nodes, 2) to understand the impact of failures on the system and the user applications at different scale, and 3) to identify and recreate fault scenarios that induce unrecoverable failures, in order to create new tests for system and application design. The faults were injected through special input commands to bring down network links, directional connections, nodes, and blades. We present extensions that will be needed to apply our methodologies of injection and analysis to the Cray XC (Aries) systems.

==> 00000-Intro.tex <==
\section{Introduction}
\label{s:intro}
%%%%%%%%%%%%%%%%%%%%%%%%


\comment{Note - revise the abstract as necessary}

\comment{Dont wordsmith for now, but feel free to add in other contributions/impacts}.

As we move to exascale, it is expected that increasing faults...blah blah blah..... We need to understand fault-to-failure
scenarios and best places to instrument/inform/mitigate. Difficult to do this in production because of intermittent failures,
lacking control to investigate variations, etc.

In previous work~\cite{jha2016analysis},
we presented fault and recovery state diagrams based on the Gemini documentation and empirical evidence
from the logs of Blue Waters. We used the log information to populate our LogDiver tool with the appropriate log lines and sequences
of events in order to be able to automatically identify fault, recovery, and failures in the recoveries. In addition, we characterized
timelines of events that occurred in production on Blue Waters. This work was constrained however to only those naturally
occurring events and to characterizations that might be tied to the component count of Blue Waters.

In this work, we extend that previous work in several ways:
\begin{itemize}
\item We expand the scenarios we can investigate by using controlled fault injection experiments.
\item We include system and application state data to assess the impact of the faults.
\item We investigate the faults and effects on a different large-scale XE platform, Cielo.
\end{itemize}

Fault injection enables us to investigate controlled complex events that may be rare.
Note however that with larger systems the potential for multiple concurrent failures and wide spread impact increases.
Control of the experiments enables us to better extract out failure-related events and log
messages from the normal system events which include components down and error messages going on.

In support of this work, we have developed a tool, HPCArrow, for causing and investigating a variety of fault scenarios.
Features of this tool include:
\begin{itemize}
\item Facile interface for injection and recovery, including control of multiple concurrent
and sequential faults
\item Underlying mechanisms for injection and recovery
\item Recording of timelines of event occurences for subsequent analysis
\end{itemize}

We analyze the resultant event data provided by Cray systems using LogDiver.
We augment the system data with network performance data collected by LDMS inorder to assess system and application
impact.

Contributions of this work are:
\begin{itemize}
\item Development of methodologies for investigating and assesssing faults and impacts through fault injection techniques
\item Implementation of those methodologies in tools
\item Investigation of concrete occurences (not a simulation) of complex fault scenarios and impacts in a large-scale system, including failures of recoveries
\item Demonstrations of these tool in characterizing complex fault scenarios
\item Recommendations for and gap analysis of notification and instrumentation to be used in HPC resilience mechanisms, based on our data-driven analysis
\item Initial extensions of this work to Aries systems.
\end{itemize}

This paper is organized as follows:
Section~\ref{s:motivation} provides motivation for this work.
Section~\ref{s:FI} describes the targetted FI scenarios and Cray's automated recovery mechanisms.
Section~\ref{s:fitool} describes our fault injection tool developed for this work.
Section~\ref{s:analysis} describes our event and impact analysis methodology and tools.
Section~\ref{s:results} presents results of the fault injection experiments.
Section~\ref{s:resilience} presents how the results of our experiments can be applied to improving resilience in HPC systems.
Section~\ref{s:aries} describes our progess in extending our work to Aries systems.
Section~\ref{s:relatedwork} presents related work.
Finally, we conclude in Section~\ref{s:conclusion}.







==> LDMS.tex <==
>\section{LDMSPlots}
\label{s:LDMSPlots}

This section is a placeholder for the LDMS~\cite{LDMSSC14} plots and related material.

As part of the experiments we ran a workload of various-sized instances of IMB~\cite{imbintel} all-to-all jobs.
IMB all-to-all exhibits nearly continuous significant traffic on the system. We
monitored a variety of network counters on all routers, and investigated the job progress
impact due to the faults and recovery processes as evinced by impacts to these counters.

Quantities monitored included traffic, stalls, and link status on the \emph{aggregated} directional links \texttt{X,Y,Z} in both \texttt{+,-} (total of 6 directions) as presented by Cray's \emph{gpcdr} interface~\cite{craygpcdr}.
Traffic is reported by the Gemini performance counters in the incoming direction. Details on these quantities can be found in ~\cite{craymmr}. Data was collected at 1 sec intervals via the Lightweight Data Metric Service (LDMS). Details of LDMS data collection on Gemini Systems, including overhead assessments demonstrating that no significant detrimental system impact are given in~\cite{NCSACUG2014,LDMSSC14}. Of relevance here is that data is collected by on-node daemons and held in memory on that node until it is overwritten by the next sample. Data is pulled from that memory location by other daemons via RDMA. If network connectively is lost, as it would be during a full-system quiesce, data points during that period are currently lost.

\comment{Where do we explain links and connections?}

While in our other XE/XK systems with more current CLE the link status did change in response to downed individual links, we did not see this on Cielo. As a result, in this paper, we concentrate here on traffic measures only.

In the Gemini network, any given router may be responsible for handling traffic both for jobs allocated to
the nodes directly attached to the router as well as for other jobs' traffic that pass through that router
along their communication path. In the Gemini network, routing is primarily deterministic. Traffic goes from first
source X to destination X, then from source Y to destination Y, then from source Z to destination Z.
The shorter of paths in the $+/-$ is taken, with various rules to handle choice of paths in case of ties.
Values plotted for any routers here are thus the aggregate of traffic handled by the router; they cannot be attributed to any particular job(s) and are subject to instantaneous demands of those jobs, including job starts and stops.

In any given case of a single link or set of links in a direction are downed, the opposite direction link from the connected
router is also affected. For example, downing the link \texttt{c9-4c0s2g0l41}, which is the directional \texttt{X-} connection to \texttt{c7-4c0s2g0l04}, also downs the inverse \texttt{X+} link. All plots thus show the routers on both ends of the connection with the upper plot being that targeted by the fault injection and the lower plot being the router at the other end of the connection.


\subsection{Link Down - no case}

\comment{Dropping this case, since we have link down and restore later. The only value here is potentially showing that
a job end might affect one of the routers and not the other and that is also in the double injection.}.

%Figure~\ref{fig:ML-c9-4c0s2} is Mike's link down case. Not in the UIUC chart. The drop out is where the injection occurred. \comment{How many points were lost during this time? NOTE: job durations varied so any given Aries traffic may vary depending on the job traffic path. In this case, some jobs may have ended when that drop out was. I havent checked yet to see what job was on nodes for the top router, which would account for at least that job's traffic dropping out (although other jobs may still be routing through that same router)}
%
%For downed individual links, traffic can continue on the other links for that direction.
%
%\texttt{c9-4c0s2g0l41} \texttt{X-} link to \texttt{c7-4c0s2g0l04}.
%
%Similar to the Link and Recover case, data is lost for 30 seconds after the injection.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[hbtp]
%\centering
%\begin{minipage}[t]{\linewidth}
%\includegraphics[width=\linewidth]{6714_GB.png}
%\end{minipage}
%\vskip -16pt
%\begin{minipage}[t]{\linewidth}
%\includegraphics[width=\linewidth]{7108_GB.png}
%\end{minipage}
%\caption{Single link down in the X- direction in the upper router (top) and in its connected router (bottom). Taking down a single link only momentarily affects the network and hence the traffic collection.
%}
%\label{fig:ML-c9-4c0s2}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





\subsection{Amanda Connection - Case 5}
Figure~\ref{fig:AC-c15-0c1s6} is Amanda's Connection case. This is number 5 in the UIUC chart. \comment{Still need to check if all the directional links come back datawise - there is a lot of overlap. Also check the start times of the jobs} \texttt{c15-0c1s6} all \texttt{X+} links to \texttt{c14-0c1s6}.

\comment{Check what UIUC says about this. In this case, data drops out for 625-700 seconds during the recovery, which is longer than would be reasonably expected.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[hbtp]
\centering
\begin{minipage}[t]{\linewidth}
\includegraphics[width=\linewidth]{4684_GB.png}
\end{minipage}
\vskip -16pt
\begin{minipage}[t]{\linewidth}
\includegraphics[width=\linewidth]{4530_GB.png}
\end{minipage}
\caption{Directional Connection Fault Injection. Amanda Connection case 5. All directional links comprising the X+ direction are downed in the upper router (top) with resultant effect in the connected router (bottom).
}
\label{fig:AC-c15-0c1s6}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Link Down and Restore - no case}

Figure~\ref{fig:MLR-c14-4c1s3} is Mike's link down case with a restore during the job. Not in the UIUC chart.
The drop out is where the injection and the restore occurred.

In both the initial injection and the restore we lose data for 30 seconds. Even for just a link down, a network throttle command
is sent to all the L0's (\comment{Do we see this in random L0's?}). This is comparable to the amount of time between the throttle and the unthrottle commands. The time given in the logs between the initial link down and the notification of the warm swap successful is several minutes.

\comment{NOTE: we did not have a case with a connection restore during the job}

\texttt{c14-4c1s3g0l03} \texttt{X-} link to \texttt{c11-3c0s4g0l46}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[hbtp]
\centering
\begin{minipage}[t]{\linewidth}
\includegraphics[width=\linewidth]{5367_GB.png}
\end{minipage}
\vskip -16pt
\begin{minipage}[t]{\linewidth}
\includegraphics[width=\linewidth]{6152_GB.png}
\end{minipage}
\caption{Single Link Down and Restore. Only one of the links comprising the X- direction are downed in the upper router (top) with
resultant effect in the connected router (bottom).
}
\label{fig:MLR-c14-4c1s3}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Mike Connection - case 23}

Figure~\ref{fig:FC-c13-3c0s4} is Mike Connection case. This is 23 in the UIUC chart.


%14:03:30 - 14:03:59, unthrottle again at 14:04:30, 14:05:03 - 14:05:34
%14:04:50 - 14:05:02, unthrottle again at 14:06:46, 14:06:47 - 14:06:48

Timing - looks generally like....we lose 120 sec pretty much starting at 760-770 (although we get an intermediate point). Then we lose again another 20-25 sec starting at 937-947. These roughly correspond to the fact that we have 2 separate throttling events, the first of which has to be redone and is therefore longer.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[hbtp]
\centering
\begin{minipage}[t]{\linewidth}
\includegraphics[width=\linewidth]{5288_GB_v2.png}
\end{minipage}
\vskip -16pt
\begin{minipage}[t]{\linewidth}
\includegraphics[width=\linewidth]{5290_GB.png}
\end{minipage}
\caption{Single Connection Fault Injection. Traffic rate vs time for the directional links of Gemini router for which all Z+ directional links were failed (top).
Traffic on all links stops while the network is quiesced and rerouted. After the rerouting, traffic resumes on all links except
for the still down Z+ links (yellow). The router connected to this one correspondingly loses traffic on its Z- links (blue).
}
\label{fig:FC-c13-3c0s4}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Mike 2 connection - no case}

Successful recovery of a double connection injection:  \texttt{c3-1c0s6} \texttt{Y-} link to \texttt{c3-1c0s6}
and \texttt{c0-0c2s2} \texttt{Y-} link to \texttt{c0-1c0s2} Figure~\ref{fig:M2C}.


\comment{same as other about the job ending check}

First injection: lose about 120 sec starting at 655, with some intermediate datapoints on the second router.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[hbtp]
\centering
\begin{minipage}[t]{\linewidth}
\includegraphics[width=0.9\linewidth]{8594_GB.png}
\end{minipage}
\vskip -13pt
\begin{minipage}[t]{\linewidth}
\includegraphics[width=0.9\linewidth]{8588_GB.png}
\end{minipage}
\vskip -13pt
\begin{minipage}[t]{\linewidth}
\includegraphics[width=0.9\linewidth]{0036_GB.png}
\end{minipage}
\vskip -13pt
\begin{minipage}[t]{\linewidth}
\includegraphics[width=0.9\linewidth]{0538_GB.png}
\end{minipage}
\caption{Double connection fault injection. Traffic rate vs time for the directional links of Gemini router.
All Y- directional links (orange) were failed (top and 3rd); the router connected to each one correspondingly loses traffic on its Y+ links (2nd and bottom)(teal).
}
\label{fig:M2C}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Second injection: lose  130-150  starting at 724. Times offset in the second router. \comment{Should we see the same hit in both routers? Is the throttle from the first one global? Would be interesting to see a non-involved router during some experiment. Do I have any overlapping data for any case? Also neighboring routers? Zoom in on time?}


\subsection{Mike Deadlock - case 31}

\comment{Redo this figure for the times. Check the start time -- is it correct? Becuse the injection would then be at 600, not at the 500 that it is closer to in the figs}

Double Injection:  \texttt{c7-1c0s0} \texttt{Y-} link to \texttt{c7-3c2s0} and
\texttt{c0-5c1s4} \texttt{X-} link to \texttt{c0-5c1s4} Figure~\ref{fig:DED}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[hbtp]
\centering
\begin{minipage}[t]{\linewidth}
\includegraphics[width=0.9\linewidth]{7424_GB_short.png}
\end{minipage}
\vskip -13pt
\begin{minipage}[t]{\linewidth}
\includegraphics[width=0.9\linewidth]{7358_GB_short.png}
\end{minipage}
\vskip -13pt
\begin{minipage}[t]{\linewidth}
\includegraphics[width=0.9\linewidth]{6334_GB_short.png}
\end{minipage}
\vskip -13pt
\begin{minipage}[t]{\linewidth}
\includegraphics[width=0.9\linewidth]{0840_GB_short.png}
\end{minipage}
\caption{Double connection fault injection. Traffic rate vs time for the directional links of Gemini router.
All Y- directional links were failed (top) and the router connected to it (2nd). All X- directional links were failed (3rd)
and the router connected to it (bottom). Issues during the recovery prevented the network from fully recovering and no further data was collected for this router and none of the jobs completed.
}
\label{fig:DED}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Makefile <==
# ACG stolen from amagela (AMA)
#This Makefile builds: XXX
#
# THE FOLLOWING TARGETS ARE GENERALLY AVAILABLE
# all:                Performs all tasks to clean, build, and install the application and documentation
# spellcheckaspell:   This runs a spell checker on all TeX files within doc/
# spellcheckhunspell: This runs a spell checker on all TeX files within doc/
# clean:              Delete the files generated from building the examples and documentation
# purge:              This does clean and also removes the resultant document
# tar:                Create a stamped, Gzip-compressed tarball within directory tar

###### USER SETTINGS ######
# TITLE:      Name of resultant documentation
TITLE:=main

###### COMPILER SETTINGS (ONLY ADMINS BELOW) ######
#COMPILERS/LINKERS
MAKPDF:=latexmk -pdf -f
CLEAN:=latexmk -c
PURGE:=latexmk -C

SPELLCHECKTARGET:=spellcheckaspell
ifeq ($(wildcard /usr/bin/hunspell),/usr/bin/hunspell)
	SPELLCHECKTARGET:=spellcheckhunspell
endif
ifeq ($(wildcard /opt/local/bin/hunspell),/opt/local/bin/hunspell)
	SPELLCHECKTARGET:=spellcheckhunspell
endif

#EXTRA VARS
LOGAPPEND:=$(shell date '+%Y%m%d_%H%M%S')

###### TARGETS ######
#default: initpurge pdf clean
#ACG perfers to call clean separately
default: initpurge pdf
pdf: $(TITLE).pdf
$(TITLE).pdf: $(TITLE).tex
%.pdf: %.tex
#	$(MAKPDF) >$*.build.log 2>&1 $<
	$(MAKPDF) $<

.PHONY: clean
clean:
	$(CLEAN)
	-find . -type f -name "*.bbl" -exec rm -f '{}' \;
	-find . -type f -name "*~" -exec rm -f '{}' \;
	-find . -type f -name "*.swp" -exec rm -f '{}' \;
	-find . -type f -name ".*~" -exec rm -f '{}' \;
	-find . -type f -name ".*.swp" -exec rm -f '{}' \;

#ACG added to get rid of pdf but not break the other calls
.PHONY: veryclean
veryclean: clean
	$(VERYCLEAN)
	-rm $(TITLE).pdf

.PHONY: initpurge
initpurge:
	-rm -f $(TITLE).pdf

.PHONY: purge
purge: clean
	$(PURGE)

.PHONY: spellcheckaspell
spellcheckaspell:
	-find . -type f -name "[0-9]*.tex" -exec aspell -c '{}' --lang=en_US --mode=tex \;

.PHONY: spellcheckhunspell
spellcheckhunspell:
	-find . -type f -name "[0-9]*.tex" -exec hunspell -t -d en_US '{}' \;

.PHONY: spellcheck
spellcheck: $(SPELLCHECKTARGET)

.PHONY: tar
tar: clean
	mkdir -p tar
	tar -czhf tar/$(TITLE)_$(LOGAPPEND).tgz $(TITLE).pdf Makefile *.tex *.bib figs


==> introduction-sj.tex <==
\section{Introduction}

As we move to exascale, the system is expected to experience much higher error rates\cite{snir2014addressing,yang2012reliability}. To overcome the \quotes{resiliency wall} \cite{yang2012reliability} in exascale systems, we need to understand fault-to-failure scenarios and identify optimal places to instrument the system for detecting and mitigating faults. Understanding fault-to-failure scenarios is difficult in production due to intermittent failures, lacking control to investigate variations, inability to recreate conditions, etc. In this work, we focus on understanding faults/failures and recoveries in the interconnection network of a supercomputer as it serves both inter-node communications and file system traffic. %The resiliency of interconnection network is fundamental to sustaining large-scale application and system. The unavailability/failure of network effects the entire system.

In previous work \cite{jha2016analysis}, we presented network failures and recovery state diagrams and showed the criticality of these failures on system and applications by providing empirical evidence of network component failures  and the failure of the triggered network recovery.  This work was constrained however to only those naturally occurring events and to characterizations that might be tied to the component count (scale) of Blue Waters. Further, presence of multiple errors and failures (as indicated by logs) made it difficult to diagnose and understand the reason for some of the recovery failures in the system.

To overcome those limitations and better understand fault-to-failure propagation in large-scale supercomputer interconnection networks, in this work we injected faults in the Cray XE platform, Ceilo. This is one of the largest fault injection study to date. Fault injection methods have been widely used to understand fault-to-failure propagation and its impact on application and system, since they provide the possibility to control fault conditions, and decide workload and instrumentation on the target system. To support our fault injection experiments, we developed \textit{HPCArrow} tool and studied the propagation of the faults in the network and tested the recovery mechanisms of the interconnection network at scale. 
%\begin{itemize}
%	\item Emulate failure scenarios to verify and extend the understanding of the fault propagation in the system
%	\item Identify error logs and conditions that lead to catastrophic failures
%	\item Investigate the effects of faults on a different large-scale XE platform, Cielo.
%\end{itemize}
%   In this work, we inject faults in the network components as network is a fundamental sub-system providing inter-communication paths between nodes and read/write traffic for the storage sub-system.  test recovery and containment capabilities of Cray XE systems 

Contribution and results of this work are summarized below \textemdash 

\begin{itemize}
	\item \textbf{Network fault injection methodology for large-scale supercomputers:} design and development of holistic fault injection and error characterization/evaluation methodology (aka \textit{HPCArrow}) to create various failure scenarios such as multiple link failures, link failures during recovery, etc. in Cray HPC interconnection networks. \textit{HPCArrow} can create complex failure scenarios that can emulate observed field-data network failure scenarios or create new ones to assess the system resiliency new failure scenarios (that are yet to be seen in the production).
	
	\item \textbf{Validation and extension of field failure data analysis:} investigation, validation and extension of failure scenarios presented in \cite{jha2017Resiliency, jha2016analysis} and establish in-dept fault-to-failure scenarios and fault propagation delays. \note{mention some of the validations or new things made in a line or two}
	
	\item \textbf{Recommendation for notification and instrumentation: } identification of critical error logs and conditions that appear during network-related failures that lead to application and/or system failures. For example, when the system is deadlocked the hardware components keep reporting  \quotes{ORB RAM Scrubbed Upper Entry}. In other cases, these error are not reported after few seconds of finished network recovery. Such complex error patterns mined using fault injection techniques can help in diagnosis and monitoring of the system.%Complex pattern mining (e.g., "recovery finished" and "ORB Scrubbed" together form a pattern) would assist in system monitoring.
	
	\item \textbf{Recommendation for future fault injection experiments:} \note{either write here or in conclusion}
 
\end{itemize}
This paper is organized as follows:
Section~\ref{s:motivation} provides motivation for this work.
Section~\ref{s:FI} describes the targetted FI scenarios and Cray's automated recovery mechanisms.
Section~\ref{s:fitool} describes our fault injection tool developed for this work.
Section~\ref{s:analysis} describes our event and impact analysis methodology and tools.
Section~\ref{s:results} presents results of the fault injection experiments.
Section~\ref{s:resilience} presents how the results of our experiments can be applied to improving resilience in HPC systems.
Section~\ref{s:aries} describes our progess in extending our work to Aries systems.
Section~\ref{s:relatedwork} presents related work.
Finally, we conclude in Section~\ref{s:conclusion}.



